Hybrid Beamforming with Reduced Number of Phase Shifters for Massive MIMO Systems

In this paper, two novel hybrid beamforming methods are proposed to reduce the cost and power consumption of hybrid beamformers with subconnected phase shifter network structure in massive multiple-input multiple-output (MIMO) systems. This is achieved by replacing some of the phase shifters with switches which, in general, are cheaper and have lower power consumption compared to phase shifters. The proposed methods and the closed-form expressions of their performance are derived according to the properties of the elements of the singular vectors of the channel matrix. In the first approach, it is shown that by combining the subconnected phase shifter network with a fully-connected switch architecture, the number of the phase shifters can be reduced up to 50\% while the spectral efficiency is preserved. Then, in order to simplify the structure of the switch network, the fully-connected switches is replaced by subconnected switch network, e.g. binary switches. The analytical and simulation results indicate that just by using 25% of phase shifters 90% spectral efficiency can be achieved. Finally, simulation results indicate that similar behavior is observed when the wireless channel is considered to be sparse or correlated.

==> Introduction.tex <==
\section{Introduction}

Massive multiple-input multiple-output (MIMO) technology with digital beamforming can increase the spectral efficiency in wireless communication systems. However, a dedicated RF chain per antenna increases the cost of this technology. To reduce the number of RF chains, hard and soft antenna selection techniques have been proposed. To perform antenna selection, a small number of RF chains are connected to a large number of antennas through a network of phase shifters/switches, known as soft/hard antenna selection \cite{MOlischAntennaselection2005Journal}. The phase shifter/switch networks are categorized as fully-connected and subconnected \cite{5GHybridlargeantenna,7445130}. In the fully-connected configuration, there is a connection from each RF chain to all of the antenna whereas, in the subconnected structure, each RF chain is connected to only a subset of the antennas. In general, performing antenna selection to achieve a high performance is a difficult problem as it requires solving a nonconvex optimization which is due to the nonconvex constraints imposed by switches/phase shifters \cite{MOlischAntennaselection2005Journal}. In the following, we review the existing work on antenna selection methods when fully-connected/subconnected structures with switches/phase shifters are used. It is noted that our performance metric throughout this paper is spectral efficiency.

Hard antenna selection has shown to be effective when Soft antenna selection, also known as hybrid beamforming, with fully-connected phase shifters network has shown to be able to achieve similar performance to that of digital beamformers \cite{SohailJornal,SpatiallySparsePrecodingAyach}. 

The drawback of this approach is that large beamforming gains cannot be achieved as only a small fraction of the antennas are used \cite{MOlischAntennaselection2005Journal,7172496,7417765}.

Phase shifters provide more flexibility and better performance compared to switches at the cost of higher power consumption \cite{HeathLetter,7445130,7370753,HeathITA2015}. 




In addition, depending on the configuration of the switch or phase shifter network, they are categorized as fully-connected and subconnected structures. In the fully-connected configuration, there is a connection from each RF chain to each antenna element, whereas in the subconnected structure each RF chain is routed to only a subset of the antennas. 

Compared to switches, phase shifters are not only more expensive, but also they have a higher power consumption \cite{HeathLetter,7445130,7370753,HeathITA2015}.


  For the fully-connected structure 

 In the soft antenna selection, also known as hybrid beamforming, the RF chains and the antennas are connected through a network of phase shifters \cite{SohailJornal,SpatiallySparsePrecodingAyach}. Such architectures are cheaper than digital beamformers and they achieve a higher spectral efficiency compared to hard selection. There are two types of phase shifter networks known as fully-connected and subconnected \cite{5GHybridlargeantenna,7445130}. It can exploit the full array gain, however, its power consumption can be very high due to the massive number of the phase shifters it requires \cite{SohailJornal,HeathITA2015,7370753,HeathLetter,7445130}. In the subconnected configuration, each RF chain is connected to a subset of antennas which results in simplicity of the circuits and lower cost, but also a lower spectral efficiency compared to the fully-connected system \cite{7445130}. In general, the design of the optimal soft antenna selection schemes is a challenging task due to the nonconvex constant modulus constraint imposed by the phase shifters \cite{SohailJornal,SpatiallySparsePrecodingAyach}.  Similar to the phase shifter networks, switch networks have fully-connected and subconnected structures. Due to the large number of switches, fully-connected configuration has high hardware complexity, insertion losses as well as crosstalk distortion \cite{7417765}. Hence, subconnected configuration for the switch network, such as binary switches, is preferred in practice despite providing less degrees of freedom in designing the antenna selector.


{\color{blue}{The performance of antenna selection techniques with fully-connected and subconnected switches was evaluated over measured massive MIMO channels at 2.6 GHz with 128 antennas at the base station \cite{7417765,7172496}. It was shown that fully-connected and subconnected switches provide a competitive performance in terms of spectral efficiency when the number of RF chains are significantly larger than the number of the users, otherwise the overall spectral efficiency will drop due to the losses in array gain. In \cite{HeathITA2015,7370753}, a comprehensive study of power and spectral efficiencies is provided for multiple millimeter wave hardware configurations. It was shown that using binary switches at the transceivers significantly improves the system simplicity and energy efficiency, however, when the number of antennas goes large, the computational complexity grows exponentially. Similar to \cite{7417765,7172496}, the results in \cite{HeathITA2015,7370753} indicate that antenna selection techniques that only rely on switches, cannot provide high sum-rates. Hence, antenna selection with switches results in high power efficiency at the cost of low spectral efficiency. On the other hand, antenna selection with phase shifters leads to in high spectral efficiency at the cost of low power efficiency. Recently, the authors in \cite{HeathLetter} bridged the two approaches by using a combination of switches and non-tunable phase shifters. This method  can reach the spectral efficiency of hybrid beamforming with fully-connected phase shifter network. While the approach in \cite{HeathLetter} requires a relatively low computational complexity as well as low power consumption, it requires a massive number of RF routes which result in a complex hardware and high levels of crosstalk \cite{7417765,5GHybridlargeantenna}. In \cite{SohailJornal}, where a fully-connected phase shifter network was considered, it was shown that by equipping each phase shifter with a switch, it is possible to reduce the power consumption of the RF beamformer by turning off almost 50\% of the phase shifters and preserve the spectral. With the motivation to reduce the power consumption of massive MIMO systems while achieving high sum-rates, we believe there is a need for investigating new techniques to jointly design the beamforming weights at the baseband, phase shifter as well as the switch networks . 

In this paper, two novel combinations of phase shifters and switches are proposed and their performance in terms of the achievable sum-rate are evaluated. To this end, first we derive the closed-form expression of the beamformer and its achievable sum-rate over uncorrelated independent and identically distributed (i.i.d.) channel when the RF beamformer has subconnected structure. This approach offers lower computational complexity and similar performance compared to the successive interference cancellation based method in \cite{7445130} when a small number of RF chains are connected to a large number of antennas. Second, based on the presented approach for the subconnected phase shifter network and using phase shifter selection technique, in \cite{SohailJornal}, for fully-connected phase shifter network, it is shown that a combination of subconnected phase shifter and fully-connected switch networks can reduce the number of the phase shifters 50\% without a performance loss over uncorrelated i.i.d. Rayleigh fading channels. The simulation results for sparse scattering and correlated Rayleigh fading channels indicate that the achievable sum-rates almost remain at the same level when the number of the phase shifters are reduced to half. However, as the proposed structure requires a fully-connected switch network, which may not be suitable for practical applications, it is desirable to substitute the complex switch network with simpler structures, for example binary switches. Hence, we present a novel beamforming method that provides a slightly lower performance, however, it requires a much simpler hardware structure. In this approach, the fully-connected switches are replaced with simple subconnected switches, e.g. binary switches. Finally, the simulation results indicate that the asymptotic closed-form expressions of the spectral efficiency provide a good approximation of the performance for moderate number of antennas and phase shifters.

This paper is organized as following, the system model and hybrid beamforming with subconnected phase shifter network are described in sections \ref{sec:SystemModel} and \ref{sec:figb}. In section \ref{sec:figc}, the proposed method for hybrid beamforming with subconnected phase shifters and fully-connected switches are presented. The analysis for the subconnected phase shifters that are connected to subconnected subconnected switch network are discussed in \ref{sec:figd}. Finally, the simulation results and conclusion are presented in sections \ref{sec:SecSR} and \ref{sec:con}. }}

\textit{Notations:} Bold capital and small letters \textbf{A} and \textbf{a} represent a matrix and a vector, respectively. $ A_{mn}$ denotes the $(m,n)$-th element of \textbf{A}, $\textbf{a}_m$ is the $m$-th column of \textbf{A} and $\textbf{A}_{1:m}$ is a matrix containing the first $m$ columns of \textbf{A}. det$( \textbf{A} )$, $\textbf{A}^\text{H}$ and trace(\textbf{A}) denote determinant, Hermitian and trace of \textbf{A}, respectively. Moreover, $\vert A \vert$ and $\angle A$ denote the magnitude and angle of complex number $A$. $\textbf{I}_m$ is an $m \times m$ identity matrix. Finally, $f_A(a)$, $F_A(a)$ and E$[A]$ denote the probability density function (pdf), cumulative distribution function (cdf) and expected value of $A$, respectively. 








==> Introduction2.tex <==
\section{Introduction}

Massive multiple-input multiple-output (MIMO) technology with digital beamforming can increase the spectral efficiency in wireless communication systems. However, a dedicated RF chain per antenna increases the cost of this technology. In order to reduce the number of RF chains, hard and soft antenna selection techniques have been proposed \cite{MOlischAntennaselection2005Journal}. In the hard selection, the RF chains are connected to the antennas by a network of switches. The drawback of this approach is that large beamforming gains cannot be achieved as only a small fraction of the antennas are used \cite{MOlischAntennaselection2005Journal,7172496,7417765}. In the soft antenna selection, also known as hybrid beamforming, the RF chains and the antennas are connected through a network of phase shifters \cite{SohailJornal,SpatiallySparsePrecodingAyach}. Such architectures are cheaper than digital beamformers and they achieve a higher spectral efficiency compared to hard selection. There are two types of phase shifter networks known as fully-connected and subconnected \cite{5GHybridlargeantenna,7445130}. In the fully-connected structure, each RF chain is connected to all the antennas as in \cite{SohailJornal,SpatiallySparsePrecodingAyach}. It can exploit the full array gain, however, its power consumption can be very high due to the massive number of the phase shifters it requires \cite{SohailJornal,HeathITA2015,7370753,HeathLetter,7445130}. In the subconnected configuration, each RF chain is connected to a subset of antennas which results in simplicity of the circuits and lower cost, but also a lower spectral efficiency compared to the fully-connected system \cite{7445130}. In general, the design of the optimal soft antenna selection schemes is a challenging task due to the nonconvex constant modulus constraint imposed by the phase shifters \cite{SohailJornal,SpatiallySparsePrecodingAyach}. Compared to switches, phase shifters are not only more expensive, but also they have a higher power consumption \cite{HeathLetter,7445130,7370753,HeathITA2015}. Similar to the phase shifter networks, switch networks have fully-connected and subconnected structures. Due to the large number of switches, fully-connected configuration has high hardware complexity, insertion losses as well as crosstalk distortion \cite{7417765}. Hence, subconnected configuration for the switch network, such as binary switches, is preferred in practice despite providing less degrees of freedom in designing the antenna selector.


{\color{blue}{The performance of antenna selection techniques with fully-connected and subconnected switches was evaluated over measured massive MIMO channels at 2.6 GHz with 128 antennas at the base station \cite{7417765,7172496}. It was shown that fully-connected and subconnected switches provide a competitive performance in terms of spectral efficiency when the number of RF chains are significantly larger than the number of the users, otherwise the overall spectral efficiency will drop due to the losses in array gain. In \cite{HeathITA2015,7370753}, a comprehensive study of power and spectral efficiencies is provided for multiple millimeter wave hardware configurations. It was shown that using binary switches at the transceivers significantly improves the system simplicity and energy efficiency, however, when the number of antennas goes large, the computational complexity grows exponentially. Similar to \cite{7417765,7172496}, the results in \cite{HeathITA2015,7370753} indicate that antenna selection techniques that only rely on switches, cannot provide high sum-rates. Hence, antenna selection with switches results in high power efficiency at the cost of low spectral efficiency. On the other hand, antenna selection with phase shifters leads to in high spectral efficiency at the cost of low power efficiency. Recently, the authors in \cite{HeathLetter} bridged the two approaches by using a combination of switches and non-tunable phase shifters. This method  can reach the spectral efficiency of hybrid beamforming with fully-connected phase shifter network. While the approach in \cite{HeathLetter} requires a relatively low computational complexity as well as low power consumption, it requires a massive number of RF routes which result in a complex hardware and high levels of crosstalk \cite{7417765,5GHybridlargeantenna}. In \cite{SohailJornal}, where a fully-connected phase shifter network was considered, it was shown that by equipping each phase shifter with a switch, it is possible to reduce the power consumption of the RF beamformer by turning off almost 50\% of the phase shifters and preserve the spectral. With the motivation to reduce the power consumption of massive MIMO systems while achieving high sum-rates, we believe there is a need for investigating new techniques to jointly design the beamforming weights at the baseband, phase shifter as well as the switch networks . 

In this paper, two novel combinations of phase shifters and switches are proposed and their performance in terms of the achievable sum-rate are evaluated. To this end, first we derive the closed-form expression of the beamformer and its achievable sum-rate over uncorrelated independent and identically distributed (i.i.d.) channel when the RF beamformer has subconnected structure. This approach offers lower computational complexity and similar performance compared to the successive interference cancellation based method in \cite{7445130} when a small number of RF chains are connected to a large number of antennas. Second, based on the presented approach for the subconnected phase shifter network and using phase shifter selection technique, in \cite{SohailJornal}, for fully-connected phase shifter network, it is shown that a combination of subconnected phase shifter and fully-connected switch networks can reduce the number of the phase shifters 50\% without a performance loss over uncorrelated i.i.d. Rayleigh fading channels. The simulation results for sparse scattering and correlated Rayleigh fading channels indicate that the achievable sum-rates almost remain at the same level when the number of the phase shifters are reduced to half. However, as the proposed structure requires a fully-connected switch network, which may not be suitable for practical applications, it is desirable to substitute the complex switch network with simpler structures, for example binary switches. Hence, we present a novel beamforming method that provides a slightly lower performance, however, it requires a much simpler hardware structure. In this approach, the fully-connected switches are replaced with simple subconnected switches, e.g. binary switches. Finally, the simulation results indicate that the asymptotic closed-form expressions of the spectral efficiency provide a good approximation of the performance for moderate number of antennas and phase shifters.

This paper is organized as following, the system model and hybrid beamforming with subconnected phase shifter network are described in sections \ref{sec:SystemModel} and \ref{sec:figb}. In section \ref{sec:figc}, the proposed method for hybrid beamforming with subconnected phase shifters and fully-connected switches are presented. The analysis for the subconnected phase shifters that are connected to subconnected subconnected switch network are discussed in \ref{sec:figd}. Finally, the simulation results and conclusion are presented in sections \ref{sec:SecSR} and \ref{sec:con}. }}

\textit{Notations:} Bold capital and small letters \textbf{A} and \textbf{a} represent a matrix and a vector, respectively. $ A_{mn}$ denotes the $(m,n)$-th element of \textbf{A}, $\textbf{a}_m$ is the $m$-th column of \textbf{A} and $\textbf{A}_{1:m}$ is a matrix containing the first $m$ columns of \textbf{A}. det$( \textbf{A} )$, $\textbf{A}^\text{H}$ and trace(\textbf{A}) denote determinant, Hermitian and trace of \textbf{A}, respectively. Moreover, $\vert A \vert$ and $\angle A$ denote the magnitude and angle of complex number $A$. $\textbf{I}_m$ is an $m \times m$ identity matrix. Finally, $f_A(a)$, $F_A(a)$ and E$[A]$ denote the the probability density function (pdf), cumulative distribution function (cdf) and expected value of $A$, respectively. 







